Automatic Firmware Emulation through Invalidity-guided Knowledge Inference (Extended Version)

Emulating firmware for microcontrollers is challenging due to the tight coupling between the hardware and firmware. This has greatly impeded the application of dynamic analysis tools to firmware analysis. The state-of-the-art work automatically models unknown peripherals by observing their access patterns, and then leverages heuristics to calculate the appropriate responses when unknown peripheral registers are accessed. However, we empirically found that this approach and the corresponding heuristics are frequently insufficient to emulate firmware. In this work, we propose a new approach called uEmu to emulate firmware with unknown peripherals. Unlike existing work that attempts to build a general model for each peripheral, our approach learns how to correctly emulate firmware execution at individual peripheral access points. It takes the image as input and symbolically executes it by representing unknown peripheral registers as symbols. During symbolic execution, it infers the rules to respond to unknown peripheral accesses. These rules are stored in a knowledge base, which is referred to during the dynamic firmware analysis. uEmu achieved a passing rate of 95% in a set of unit tests for peripheral drivers without any manual assistance. We also evaluated uEmu with real-world firmware samples and new bugs were discovered.

==> Implement.tex <==
\vspace*{-3mm}
\section{Implementation}
\vspace*{-2mm}
\label{sec:implement}
We have developed a \sys prototype based on S2E version 2.0,
a QEMU-based concolic execution tool for program analysis.
% which has integrated the concrete and symbolic execution engine together.
S2E provides tens of useful plugins and APIs for analysts
to use for customized analysis. Therefore, \sys
can directly benefit from the open-source community.
However, the latest S2E does not support the ARM architecture~\cite{armsupport}. 
ARM support was dropped due to the switch to the KVM interface.
This limitation imposes considerable engineering
challenges for us.

Particularly,
ARM MCUs exhibit some specifics that make them incompatible with the canonical KVM interface.

% Particularly, the new S2E
% exclusively exposes a KVM interface to communicate with the QEMU for
% hardware emulation.
% However, 

We first extended S2E to support ARM MCUs with a tweaked KVM interface. 
% we first enhances S2E capability to handle ARM \cm devices.
Then we implemented the proposed knowledge extraction algorithm via three S2E plugins, namely \texttt{KnowledgeExtraction}, \texttt{InvalidStateDetection} and \texttt{InterruptControl}.
They are responsible for
extracting the \kb from the firmware via symbolic execution,
detecting the invalid execution states,
and raising interrupts, respectively.
Finally, we integrate the AFL fuzzing tool into
\sys via another plugin \texttt{FuzzerHelper}.
New components can also be easily added as plugins to
enhance our prototype.
% In this regard, 
Attributed to S2E, \sys is an extensive 
framework for MCU firmware analysis.
In total, 
we contributed more than 800 lines of code (LoC) to
extend S2E with ARM \cm support.
% including XXXX lines C code for QEMU modification and XXX lines C++ code for ARM \cm emulation and dynamic translation instrumentation integrating into S2E.
The four plugins are completed with 2,695, 794, 311, and 480 LoC, respectively.
% \gl{ add DMA plugin or not ?}
% Then, we write XXX for "RejectionsDetection" plgin used to detect the rejection conditions; and XXX lines for "PeripheralModelKBExtraction" for peripheral registers cache and match, and XXX lines for other functions such as phrase switch, log assistant, active external interrupts trigger and path selection.

% In total,
% we contributes XXX lines for S2E ARM \cm support
% including XXXX lines C code for QEMU modification and XXX lines C++ code for ARM \cm emulation and dynamic translation instrumentation integrating into S2E.
% Then, we write XXX for "RejectionsDetection" plgin used to detect the rejection conditions; and XXX lines for "PeripheralModelKBExtraction" for peripheral registers cache and match, and XXX lines for other functions such as phrase switch, log assistant, active external interrupts trigger and path selection.


% To add arm support for S2E, we first move fore-end TCG of ARM in vanilla ARM QEMU CPU emulation and add XXXX lines C code to make it is able to communicate with S2E core. 
% Then we add XXX lines C code for cortex-m kvm mode support for vanilla QEMU and add corresponding XXX lines C code for necessary emulated ARM cortex-m KVM interfaces.
% For automatic peripheral modeling, we write XXX for LoopDetection plgin used to detect the path switch conditions we set in Section X, we use XXX lines for path selection, XXX lines for peripheral mode cache and match, and XXX lines for other plugins such as log assistant, external interrupts trigger. 
% At last, we also use AFL v256b version to generate fuzzing input to our current prototype, which has no built-in support or
% awareness of MCU firmware.

\vspace*{-3mm}
\subsection{Cortex-M Support for S2E}
\vspace*{-2mm}
\label{sec:armsupport}

Since version 2.0, the code base of S2E has been refactored to decouple the hypervisor from the core symbolic execution engine.
In particular, a shared library (\texttt{libs2e}) intercepts and emulates calls to \texttt{/dev/kvm} to provide symbolic execution capabilities.
Technically, S2E borrows the traditional
dynamic binary translation (DBT) implementation of QEMU,
and combines it with the KLEE symbolic execution engine
to emulate the guest CPU in \texttt{libs2e.so}.
Then, by exposing a KVM-compatible interface, 
an existing KVM client such as QEMU can
control guest machine execution and emulate virtual peripherals to the guest CPU.
Since the KVM interface is relatively stable in the Linux kernel,
S2E can be easily ported to other KVM-based hypervisors, or
keep updated to its official upstream hypervisor (QEMU),
which constantly supports new peripherals.
On the contrary, the core symbolic execution part (including DBT and KLEE)
is seldom updated.
% \gl{should delete the following statements. The S2E update TCG backend this year but keep the forend in libcpu still as version 1.0}
% For example, the Tiny Code Generator (TCG), which is the DBT engine
% of S2E, was extracted from QEMU 1.0 and never updated since then.


% \sys follows the design of S2E. 
% Therefore, the two major components are
% CPU emulation which implemented as \texttt{libs2e} and
% the hardware emulation which is implemented by QEMU.
% They are bridge by the KVM interface.


% while the upstream QEMU has upgraded TCG to version 5.0 at the time of writing.


Although the benefit of switching to the KVM interface
is obvious, it sacrifices broad architecture support
because not every architecture can be easily managed by the KVM interface.
Currently, S2E 2.0 only supports the x86/x86-64 architecture and
general support for ARM remains a lot of work to do~\cite{armsupport}.
% \footnote{We acknowledge that KVM also supports ARM cortex-A series CPUs. The reason why S2E does not support ARM cortex-A architecture remains unknown to us.}
To implement ARM \cm support for S2E,
there are two main tasks involved.
The first task is to port the DBT for ARM
to \texttt{libs2e.so} so as to emulate ARM MCUs.
The second task is to make the emulated CPU
accessible via the KVM interface.



% To decouple S2E with specific client hypevisors (e.g., QEMU),
% the S2E has been fundamentally changed its framework from 2.0 version.
% In a nutshell, it use a shared library that integrates the dynamic binary translation (DBT) implemented by QEMU with KLEE symbolic execution engines as a KVM-compatible CPU emulator
% as shown in the figure~\ref{fig:arch}, 
% to intercepts and emulates calls to KVM interfaces instead of actual KVM.



% Thus, to add KVM ARM Cortex-M extensions for S2E,
% we first need to add \cm KVM Mode Support for QEMU and add \cm CPU emulation to the S2E.

\vspace*{-2mm}
\subsubsection{CPU Emulation}
This task is relatively straightforward because the upstream QEMU
already supports the ARM architecture, including ARM \cm series MCUs.
We directly extracted the corresponding logic implemented in the \texttt{libcpu} of QEMU that decodes the ARM instruction and further interfaced it with the TCG front-end compiler.
Due to the nature of intermediate representation,
the back-end of TCG was largely untouched.
Then we made necessary modifications
to facilitate the communication with the core S2E logic and
to generate events that are used by the callback functions in the plugin framework.
These are essential for \sys to 
place hooks at translation block boundaries and other
interesting execution points.

 
 
% We first copy ARM CPU emulation and TCG code corresponding to the same version of vanilla QEMU (i.e., 1.0) used by S2E X86 emulation.
% We instrumented and exposed necessary data structure and low-level events used by S2E
% in ARM \cm CPU emulation and translation such as tracing start and end of one translation block, hooking MMIO read/writes 
% so as to communicate with S2E symbolic execution and event-based plugin framework.
% At last, we also need to mark which registers and memory regions in virtual CPU state can held symbolic value, etc.
% To be specific,
% we set all CPU core registers except for R15(PC) and whole RAM can store symbolic value. 
% If firmware try to jumps to the address with symbolic value,
% the S2E will concretize the symbolic value based on its current path constraint.
\vspace*{-2mm}
\subsubsection{KVM Interface Implementation}

In essence, S2E provides a virtual CPU (vCPU) capable of symbolic execution, and QEMU manages the vCPU via KVM interfaces.
Ideally, we only need to implement all the canonical the KVM interfaces, for example, \texttt{KVM\_RUN}
to allocate a vCPU and \texttt{KVM\_SET\_USER\_MEMORY\_REGION} to allocate a RAM region.
% By implementing them
% on top of the emulated ARM \cm CPU,
% The concrete implementation is kept transparent to QEMU.
However, ARM \cm CPUs exhibit many specifics that
render the implementation more challenging.
Sometimes, a dedicated interface has to be added
for QEMU to fully manage the ARM \cm vCPU.
This necessitates the modification to QEMU.
We summarize the major changes we made as follows.


% The ARM \cm devices are designed for
% cost and energy-efficient microcontrollers, which do not support
% hardware-assisted virtualization.
% Therefore, the 
% KVM-friendly.
% To add ARM Cortex-M support for S2E,


% Naturally,
% Kernel-based Virtual Machine (KVM) is a full virtualization solution on x86 hardware or 64-bit ARM architecture,
% thus Qemu also does not support KVM mode for ARM CPU emulation on X86 CPU either.

% We first change the compile configure to enable Qemu to run the
% ARM-based firmware in KVM mode instead of TCG mode.
% Thus, we can reuse the general KVM mode deployment for 64-bit ARM architecture like
% building a virtual machine, creating a virtual CPU and running instructions with the VCPU.
% Then, we revise all specific KVM interfaces related VCPU to make it compatible with \cm and S2E.
% The major changes are as follow:

\paragraph{Register Initialization.}
On x86 CPUs, all the core registers are initialized into pre-defined values at reset. For example, the PC register at reset is fixed at \texttt{0xFFF0} and the CS register is at \texttt{0xF000}. However, some ARM registers
are initialized based on the ROM content, which in turn
is a part of firmware image.
For example,
the initial stack pointer is loaded with the first four bytes
from the address {0x00} in ROM while the PC is loaded with the following
four bytes~\cite{armv7m}.
Since this information is only available to the QEMU,
we added another KVM interface \texttt{KVM\_SET\_CORTEX\_M\_REGS} to pass the values of these registers to the CPU emulation.

\paragraph{Memory Registration.}
S2E keeps track of multiple execution states simultaneously. 
To switch between states, it needs to save the previous state and restore the next one.
S2E uses a custom KVM API called \texttt{KVM\_MEM\_FIXED\_REGION} to register the properties of
a memory region for the guest, including the virtual address on the host, the size as well as a shareable flag.
Only memory regions registered under \texttt{KVM\_MEM\_FIXED\_REGION} can be properly managed by S2E during execution state switches. 
In \sys, the user needs to specify the regions for ROM and RAM so that
we can properly register them with \sys.
For ROM regions, we set them as shareable so that each execution state
accesses the same read-only copy of the code.
For RAM regions, we set them as non-shareable so that each state
works on its own copy.

\paragraph{System State Synchronization.}
Apart from memory, peripheral and interrupt states also need to be maintained for each execution state.
In \sys, we use the custom KVM interface \texttt{KVM\_DEV\_SNAPSHOT} to
save and restore the state of system peripherals and interrupts, such as
\textit{nested vectored interrupt controller} (NVIC) and \textit{system control block} (SCB).


% During initialization, to enable S2E initialize and manage per-state memory regions,
% we also need to registers guest physical memory to the S2E via \texttt{KVM\_MEM\_FIXED\_REGION} API, specifying the host virtual address, the size of the allocated region and shared flag (whether the given memory chunk may be shared among all execution paths).
% For \cm specific, we register the code segment (i.e., ROM) as shared memory regions
% since all paths only need to read from it and the data segments (i.e., RAM) as individual memory region for each path.
% According to the memory map of ARM \cm, we set 0x0 to 0x1fffffff as code segment and 0x2000000 to 0x4000000 by default.
% However, the actual memory space firmware used is much smaller than that.
% Thus,
% we also allow the user to customize memory regions (i.e., the mapping range of RAM/ROM) according the its datasheet.
% Usually, the chip information can be obtained from the
% product description. With the chip information, it is not hard
% to find out the datasheet or manual of the chip.




% S2E maintains the CPU registers and Memory in different path by it own and leverages the QEMU to save and restore externals device states to/from specific memory via \texttt{KVM\_DEV\_SNAPSHOT} API like VGA.
% Corresponding to \cm, we need to save system peripherals state for each path.
% In addition,
% during runtime, firmware will dynamically
% disables and re-enables or reset the priority level of interrupts as needed.
% Thus, we also need to save the
% states and priority levels of all interrupts for each path to keep whole environment consistent.
% To be specific,
% when forking or switching to a new execution path,
% we force exit \texttt{KVM\_RUN} and use \texttt{KVM\_DEV\_SNAPSHOT} API to saving/restore these states.
% Note that 
% since S2E prohibits symbolic data leaking into the KVM client and therefore the KVM API does not need support for symbolic data exchange.
% We inherit this design, since typically the system peripherals and interrupt state also does not need to handle symobolic data for our propose.



% \begin{enumerate}
% \item \textbf{Register Initialization.}


% Before running firmware \cm,
% there are several necessary register need to be configured at first.
% For example,
% Vector Table Offset Register (VTOR) contains the start address of vector table which is usually at the header of the firmware.
% The emulator need to get the
% reset value of the main stack pointer (MSP) and the start address from vector table, and the last bit of start address also indicate the 
% instruction set (i.e., thumb or arm) used by firmware.
% Thus after QEMU reading the header of the firmware and initialize the 
% special registers,
% we create a new KVM-compatible interfaces named \texttt{KVM\_SET\_CORTEX\_M\_REGS} to sync values of these registers to S2E CPU emulation.
% In case some firmware does not contain the bootloader which store the vector table and initialization code,
% we also allow the user to set VTOR, MSP and entry address via configure file.


% \item \textbf{Memory Registration.}
% During initialization, to enable S2E initialize and manage per-state memory regions,
% we also need to registers guest physical memory to the S2E via \texttt{KVM\_MEM\_FIXED\_REGION} API, specifying the host virtual address, the size of the allocated region and shared flag (whether the given memory chunk may be shared among all execution paths).
% For \cm specific, we register the code segment (i.e., ROM) as shared memory regions
% since all paths only need to read from it and the data segments (i.e., RAM) as individual memory region for each path.
% According to the memory map of ARM \cm, we set 0x0 to 0x1fffffff as code segment and 0x2000000 to 0x4000000 by default.
% However, the actual memory space firmware used is much smaller than that.
% Thus,
% we also allow the user to customize memory regions (i.e., the mapping range of RAM/ROM) according the its datasheet.
% Usually, the chip information can be obtained from the
% product description. With the chip information, it is not hard
% to find out the datasheet or manual of the chip.




% \item \textbf{System State Synchronization.}
% The S2E maintain the CPU registers and Memory in different path by it own and leverages the QEMU to save and restore externals device states to/from specific memory via \texttt{KVM\_DEV\_SNAPSHOT} API like VGA.
% Corresponding to \cm, we need to save system peripherals state for each path.
% In addition,
% during runtime, firmware will dynamically
% disables and re-enables or reset the priority level of interrupts as needed.
% Thus, we also need to save the
% states and priority levels of all interrupts for each path to keep whole environment consistent.
% To be specific,
% when forking or switching to a new execution path,
% we force exit \texttt{KVM\_RUN} and use \texttt{KVM\_DEV\_SNAPSHOT} API to saving/restore these states.
% Note that 
% since S2E prohibits symbolic data leaking into the KVM client and therefore the KVM API does not need support for symbolic data exchange.
% We inherit this design, since typically the system peripherals and interrupt state also does not need to handle symobolic data for our propose.
% \end{enumerate}



\vspace*{-2mm}
\subsection{\texttt{InvalidStateDetection} Plugin}
\vspace*{-2mm}
The \texttt{InvalidStateDetection} plugin
implements the invalid state detection function mentioned
in Section~\ref{sec:rejection}.
S2E exposes ready-to-use APIs to instrument
the firmware during dynamic binary translation.
We leverage these APIs to identify invalid execution states at runtime.
When an invalid execution state is detected,
this plugin generates a custom event named \texttt{onRejectionDection} to notify \sys.
% so that the corresponding cache policy can be upgraded or
% the execution can be rolled back to another branch. 

% We add a specific plugin to detect the following rejection conditions.
% If one of condition meets,
% we export a custom event named \texttt{onRejectionDection} to notify path selector that current path need to be switched.


% \begin{enumerate}[label = \bfseries INV\arabic*, leftmargin = 0pt, listparindent  = 15 pt]
% \begin{enumerate}[label = \bfseries INV\arabic*, leftmargin = 28pt,]
\begin{itemize}
\item \textbf{Infinite Loop.} The plugin keeps records of the control flow for each execution path.
If it observes repeated cycles in the control flow,
a loop is detected.
To further confirm an infinite loop, the plugin also 
makes sure that the processor registers are the same
in each loop.
If a register contains symbolic values, \sys solves them to concrete ones
and make the comparison.
\sys only monitors infinite loops that occurred within
the last few translation blocks.
This number is denoted as \texttt{BB\#\_INV1} and
the default value is 30 based on our empirical study.
\texttt{BB\#\_INV1} cannot be too large for two reasons.
First, monitoring a long control flow history is time-consuming.
Second, it could mistakenly recognize the main logic of the firmware as
invalid, because the main logic of the firmware is indeed
implemented in an infinite main loop.
Fortunately, the length of the repetend in the main loop 
is often much larger than that in an invalid infinite loop.
Setting \texttt{BB\#\_INV1} to
30 effectively separates them.
When an invalid infinite loop is detected,
a custom \texttt{onRejectionDection} event is raised.



\item \textbf{Long Loop.}
We use the same strategy to detect loops as is done in INV1.
% To figure out if a loop is finite, 
% the plugin observes registers with concrete values in execution states with the same PC value.
% If there is an increasing or decreasing register,
% a finite loop is detected.
The plugin further counts the number of repeated cycles.
If it exceeds an adjustable value,
the plugin confirms a long loop.
The adjustable value is denoted as \texttt{BB\#\_INV2} and
we set it as 2,000 by default based on our empirical study.
The plugin emits an \texttt{onRejectionDection} event when a long loop
is detected and the loop is not executed in the pure concrete
execution mode. This avoids falsely
detecting loops in libc
functions such as \texttt{memcpy} and \texttt{memset} as invalid. 


% Similar with infinite loop, if we found there are only one register successively increase or decrease as fix interval in a execution cycle, we count the run times of the execution cycle.
% When the count value exceeds user defined (we use 1,000 as default),
% we considers the execution is in a long loop.
% Also,
% we only emit \texttt{onRejectionDection} event when the long loop has at least one translation block is in symbolic mode.


\item \textbf{Invalid Memory Access.}
If the execution accesses memory regions that are not mapped in the ROM, RAM, system regions or external peripheral regions,
an \texttt{onRejectionDection} event is emitted.



\item \textbf{User-defined Invalid Program Points.}
We also allow analysts to specify program points
that are considered invalid.
When the execution reaches any of these points,
the plugin emits an \texttt{onRejectionDection} event. 


\end{itemize}
%\paragraph{INV1~--~Infinite Loop.}

% We maintain the runtime execution states via
% dynamic binary translation instrumentation.

% cause false positive.
% This is because the main logic of a firmware is typically implemented
% in an infinite loop with long repetends,
% and \sys might recognized it as invalid.
% However, more translation blocks are needed in each loop, compared
% with an invalid-state infinite loop which has only a few translation blocks in a loop.
% Finally, the plugin triggers a custom \texttt{onRejectionDection} event
% when there is a state containing symbolic values inside the infinite loop.


% Since most firmware finally falls into a infinite loop for main functions,
% we only detect the infinite loop within
% 30 translation blocks by default (which number can also be redefined by user).
% This design choice is proven quite efficient and accurate
% in our evaluation for real-world firmware. 
% In contrast, a finite loop must have a
% concrete counter register that controls loop termination condition.
% In addition, we also record the execution mode of each block, and only trigger \texttt{onRejectionDection} event when the infinite loop has at least one translation block is in symbolic mode.


% execution state is repeated in cycle
% we regard the current execution state in an infinite loop.
% To determine
% whether the execution state is repeated in cycle,
% we consider all registers (including program counter) in each translation block in the cycle.
% For the register stores symbolic value, we
% solve it depending on its current path constraint.
% Sometimes there is more than one concrete value that meets the constraint expression,
% we choose the first smallest positive integer to keep the solved value deterministic.
% Since most firmware finally falls into a infinite loop for main functions,
% we only detect the infinite loop within
% 30 translation blocks by default (which number can also be redefined by user).
% This design choice is proven quite efficient and accurate
% in our evaluation for real-world firmware. 
% In contrast, a finite loop must have a
% concrete counter register that controls loop termination condition.
% In addition, we also record the execution mode of each block, and only trigger \texttt{onRejectionDection} event when the infinite loop has at least one translation block is in symbolic mode.


% \paragraph{INV1~--~Infinite Loop.}
% The plugin keeps records of the control flow for each execution path.
% If it observes repeated cycles in the control flow,
% a loop is detected.
% To further confirm an infinite loop, the plugin also 
% makes sure that the processor registers are the same
% in each loop.
% If a register contains symbolic values, \sys solves it to a concrete value
% and make the comparison.
% \sys only monitors infinite loops that occurred within
% the last few translation blocks.
% This number is denoted as \texttt{BB\#\_INV1} and
% the default value is 30 based on our empirical study.
% \texttt{BB\#\_INV1} cannot be too large for two reasons.
% First, monitoring a long control flow history is time-consuming.
% Second, it could recognize the main logic of the firmware as
% invalid, because the main logic of the firmware is indeed
% implemented in an infinite main loop.
% Fortunately, the length of the repetend in the main loop 
% is often much larger than that in an invalid infinite loop.
% Setting \texttt{BB\#\_INV1} to
% 30 effectively separates them.
% When an invalid infinite loop is detected,
% a custom \texttt{onRejectionDection} event is raised.


% \paragraph{INV2~--~Long Loop.}
% We use the same strategy to detect loops as is done in INV1.
% The plugin further counts the number of repeated cycles.
% If it exceeds an adjustable value,
% the plugin confirms a long loop.
% The adjustable value is denoted as \texttt{BB\#\_INV2} and
% we set it as 2,000 by default based on our empirical study.
% The plugin emits an \texttt{onRejectionDection} event when a long loop
% is detected and the loop is not executed in the pure concrete
% execution mode. This avoids falsely
% detecting loops in libc
% functions such as \texttt{memcpy} and \texttt{memset} as invalid. 


% % Similar with infinite loop, if we found there are only one register successively increase or decrease as fix interval in a execution cycle, we count the run times of the execution cycle.
% % When the count value exceeds user defined (we use 1,000 as default),
% % we considers the execution is in a long loop.
% % Also,
% % we only emit \texttt{onRejectionDection} event when the long loop has at least one translation block is in symbolic mode.


% \paragraph{INV3~--~Invalid Memory Access.}
% If the execution accesses memory regions that are not mapped in the ROM, RAM, system regions or external peripheral regions,
% an \texttt{onRejectionDection} event is emitted.



% \paragraph{INV4~--~User-defined Program Points.}
% We also allow analysts to specify program points
% that are considered invalid.
% When the execution reaches any of these points,
% the plugin emits an \texttt{onRejectionDection} event. 





% set start address of the basic block or function as kill points. 
% If the execution jumps into keep point, we will invoke the \texttt{onRejectionDection} event.



% \begin{enumerate}
% \item \textbf{Infinite Loop.}
% We maintains the runtime execution states via
% dynamic binary translation instrumentation.
% If we found the execution state is repeated in cycle
% we regard current path is in an infinite loop.
% To determine
% whether the execution state is repeated in cycle,
% we consider all registers (including program counter) in each translation block in the cycle.
% For the register stores symbolic value, we
% solve it depending on its current path constraint.
% Sometimes there is more than one concrete value that meets the constraint expression,
% we choose the first smallest positive integer to keep the solved value deterministic.
% Since most firmware finally falls into a infinite loop for main functions,
% we only detect the infinite loop within
% 30 translation blocks by default (which number can also be redefined by user).
% This design choice is proven quite efficient and accurate
% in our evaluation. 
% In contrast, a finite loop must have a
% concrete counter register that controls loop termination condition.
% In addition, we also record the execution mode of each block, and only trigger \texttt{onRejectionDection} event when the infinite loop has at least one translation block is in symbolic mode.

% \item \textbf{Long Loop.}
% Similar with infinite loop, if we found there are only one register successively increase or decrease as fix interval in a execution cycle, we count the run times of the execution cycle.
% When the count value exceeds user defined (we use 1,000 as default),
% we considers the execution is in a long loop.
% Also,
% we only emit \texttt{onRejectionDection} event when the long loop has at least one translation block is in symbolic mode.


% \item \textbf{Invalid PC.}
% If execution need to access unmap memory region (neither in ROM, RAM, system and external peripheral memory regions),
% we also consider the current path need to be switched and trigger the \texttt{onRejectionDection} event.



% \item \textbf{User-defined Kill Point.}
% We also allow user to set start address of the basic block or function as kill points. 
% If we find the execution jumps into keep point, we will invoke the \texttt{onRejectionDection} event.

% \end{enumerate}


\vspace*{-3mm}
\subsection{\texttt{KnowledgeExtraction} Plugin}
\vspace*{-2mm}
The \texttt{KnowledgeExtraction} plugin strictly
follows the logic of Algorithm~\ref{alg:learning}.
Since S2E plugins are event-driven,
we detail how to handle some important events.




% we detail our implementation by
% explaining the most relevant events that influence the workflow.

% We detail how to automatically cache peripherals registers response values into knowledge base.
% As we mentioned in Section~\ref{},
% we keep assigning a new symbolic variable for each read operation,
% unless finding a match already saved in our knowledge base.
% At the same time, we also record corresponding execution context information for all cache type including
% hash of current function parameters, caller function, hash of last writing value to the same register and unique identity number as the symbol name.
% For example, when firmware read a value from the data register of UART which MMIO address is \texttt{0x42000818},
% we return a new symbol named as
% \texttt{0x42000818\_0x1a44\_0xeba98839680ab4e6\_1393}.

% Next,
% we need to get the concrete values that lead to expected branch targets, and determine its cache type. 
% Finally, we also need to insert and revise the value when execution meets and branch or switch to anther path.
% We achieve that through hooking the following events.


\paragraph{onRejectionDection.}
When this event is raised by the \texttt{InvalidStateDetection} plugin,
the \texttt{KnowledgeExtraction} plugin 
selects the next execution target and
raises an \texttt{onStateSwitch} event,
which is handled by S2E to prepare execution state
switching.
According Algorithm~\ref{alg:learning},
the target execution state is 
chosen from unexplored branch targets.
% , branch targets that are not fully upgraded or ancestor's branches.

\paragraph{onFork.}
This event is raised when the execution engine meets a branch decided
by a symbolic expression.
To handle it, our plugin 
solves the symbolic expression 
to get concrete values leading to each branch target.
The concrete values are then inserted into the \kb.
Specifically, if no existing entry is found, the plugin
directly inserts it as a new entry.
Otherwise, it checks if the new entry conflicts with
an existing entry and upgrades
the caching type of the corresponding peripheral register
if so.

% In addition, when execution engine runs in external interrupts,
% we directly insert the value the lead to both branch target in our knowledge base and marks it as \tirq type. 


% We maintain the value of each branch target binding with its execution context information stored in its original the symbol name.
% Therefore 
% % we save these concrete values binding to its execution context information (which are stored in the symbol name).
% % Then,
% % when a new \texttt{onFork} event emits,
% we can compare value and it context information of last branch target with the entry in our knowledge base when the execution meets a new branch.

% If no corresponding entry is found, we insert a new entry in the knowledge base.
% If corresponding entry already exists, but the value is conflict with the record, we upgrade entry type (e.g., from \tone to \ttwo) to change the cache strategy of the entry.
% In addition, when execution engine runs in external interrupts,
% we directly insert the value the lead to both branch target in our knowledge base and marks it as \tirq type. 





% we first follow the DFS algorithm to choose next candidate path. 
% If this path has not been executed, we directly switch to this path.
% Once this path has been executed, we select the path 
% based on the type of entry value that leads to last branch target.

% \paragraph{onStateSwitch:}
% Our plugin receives this event when the execution just switches
% from one execution state to another and is about
% to run the target state.

% Since we only switch the path when they meets our invalid states,
% that means the we should use the concrete values that lead to the branch target in the another path.
% Thus, every time S2E switches to another path,
% we do the same with \textit{onFork} event in normal mode.
% If execution switches path in interrupts, we just remove concrete values that lead to the wrong branch target in last path.



% \paragraph{onForkDecide}
% This event will trigger when execution meets a branch and we add a optional parameter to select default branch target.
% To be specific.
% we generate a bool rand value for branch target selection when firmware runs in interrupts, 
% but keep condition true in normal mode.
\vspace*{-3mm}
\subsection{\texttt{InterruptControl} Plugin}
\vspace*{-2mm}
Although QEMU has implemented
a virtual interrupt controller (\ie~NVIC) for ARM \cm MCUs,
which could be used to dispatch and respond to interrupts,
this function is largely limited to implementing
system peripherals such as \textit{SYSTICK},
because QEMU does not know when to fire interrupts for
custom-made peripherals.


% However, 
% Qemu do not emulate any MCU peripherals, 
% no external peripherals interrupts are fired
% when using them to run a firmware, despite that the firmware
% may crash or stall for other reasons before it gets ready for
% servicing interrupts.

For deterministic replay of interrupt sequences,
% , and arbitrary timings to be specified for emulators to fire interrupts
our prototype follows a similar interrupt firing strategy as \ppim.
It detects activated interrupts and 
delivers interrupts in a round-robin fashion at a
fixed interval defined by the user.
As empirical values, in our evaluation,
we set the interval to be once every 2,000 basic blocks
during the knowledge extraction phrase and once every 1,000 basic blocks during the analysis phase.
To find out which interrupt is activated,
the plugin checks the NVIC
\textit{Interrupt Set Enable Register} (ISER).
To deliver an interrupt, the plugin sets the corresponding
bit of the NVIC \textit{Interrupt Status Pending Register} (ISPR).


% We use Qemu \texttt{KVM\_IRQ\_LINE} API to inject the interrupts in CPU emulation.
% \texttt{armv7m\_nvic\_set\_pending} 
% \texttt{armv7m\_nvic\_complete\_irq}
% \texttt{armv7m\_nvic\_acknowledge\_irq}
% \texttt{armv7m\_nvic\_get\_active\_external\_irq}
% In addition, during runtime, 
% firmware only dynamically a handful interrupts
% enables interrupts as needed.
% If we
% fires an unused or disabled interrupt, firmware execution will also
% stall or crash because firmware commonly uses a simple dead
% loop as the default handler for unused interrupts.
% Thus, before setting a interrupt trigger,
% we first read current
% \texttt{NVIC\_ISERx} and \texttt{NVIC\_ICERx} registers
% which indicates current active interrupts


% S2E introduces ∼6× runtime overhead over vanilla QEMU when
% running in concrete mode due to checks for accesses to symbolic
% memory, and ∼78× in symbolic mode due to LLVM
% interpretation and symbolic constraint solving.
% Overall,
% we slow that the clock frequency of \cm system timer (\texttt{SYSTICK}) 20 times during knowledge extraction phrase. 
% we also force exit the execution loop to check every interrupt firing tb interval in case execution may get stuck.


% However,
% the NVIC can support up to 240 external interrupts with up to 256 different priority levels that can be dynamically reprioritized.
% It supports both level and pulse interrupt sources. 
% The processor state is automatically saved by hardware on interrupt entry and is restored on interrupt exit. 


